Is Stack Overflow Obsolete? An Empirical Study of the Characteristics of ChatGPT Answers to Stack Overflow Questions

Q&A platforms have been crucial for the online help-seeking behavior of programmers. However, the recent popularity of ChatGPT is altering this trend. Despite this popularity, no comprehensive study has been conducted to evaluate the characteristics of ChatGPT's answers to programming questions. To bridge the gap, we conducted the first in-depth analysis of ChatGPT answers to 517 programming questions on Stack Overflow and examined the correctness, consistency, comprehensiveness, and conciseness of ChatGPT answers. Furthermore, we conducted a large-scale linguistic analysis, as well as a user study, to understand the characteristics of ChatGPT answers from linguistic and human aspects. Our analysis shows that 52% of ChatGPT answers contain incorrect information and 77% are verbose. Nonetheless, our user study participants still preferred ChatGPT answers 35% of the time due to their comprehensiveness and well-articulated language style. However, they also overlooked the misinformation in the ChatGPT answers 39% of the time. This implies the need to counter misinformation in ChatGPT answers to programming questions and raise awareness of the risks associated with seemingly correct answers.

==> sections/Analysis.tex <==
\section{Methodology}

To assess the quality and correctness of ChatGPT's answers to SO questions, we used a standard NLP data labeling process ~\cite{rodrigues2014sequence,xu2020review} to label the ChatGPT answers. 

Over the course of 5 weeks, three authors met 6 times to generate, refine, and finalize the codebooks to annotate the ChatGPT answers. 
First, the first two authors familiarized themselves with the data. Each author independently annotated 5 ChatGPT answers and took notes about their observations. The two authors met to review their annotations and notes and came up with 5 aspects they wanted to assess---{\em Correctness}, {\em Consistency}, {\em Comprehensiveness}, {\em Conciseness}, and {\em Usefulness}. 
In the next step, they revisited the previous 5 ChatGPT answers to generate the initial codebook spanning the 5 assessment aspects. 

There were conflicts for 3 out of 5 of these categories. The first two authors resolved the conflicts by deciding to use 3-point and 5-point scales for two of the categories and feature-based scales for the rest of them.

% \todo{just say that you decide to use a 7-point scale.}
% \todo{mention that you have some disagreement on some answers. It would be great if you can have the number of disagreements here.}
%At this step, there were conflicts on the decision to use feature-based vs. point-based codes for each of the categories. There was consensus between Authors 1 and 2 about using point-based code for Usefulness, Comprehensiveness, and feature-based code for Correctness and Inconsistency. However, disagreement persists on whether to use the point or feature-based code for Conciseness. Which the two authors decided to discuss with Author 3.  

In the 2nd meeting, the first two authors met another co-author to resolve the disagreements and refine the codebook.  %Authors 1 and 2 annotated the previous 5 ChatGPT answers line-by-line and developed the initial codebook with common codes they observed in the 5 categories. 
At the end of this step, the refined codebook contains 26 codes in the 5 categories. 

The first two authors then moved on to annotate 20 new ChatGPT answers independently with the refined codebook. 
The codebook was refined further during this annotation step and was extended to 31 codes in 5 categories. 
After this step, they met again to discuss the annotations and refine the codebook even further.  
%Together, they reviewed 5 answers annotated by each of them. 
They carefully reviewed each annotation in the answers and compared them with the codebook to decide (1) if the annotations were correct, (2) if there was a better code to describe a group of annotations, and (3) if there was an opportunity to merge redundant codes.
%Using these three criteria, they identified the conflicts. 
\new{At this point, Fleiss's kappa score is 0.45 and Krippendorff's Alpha is 0.22.} The two authors resolved the conflicts either by merging or deleting codes, modifying definitions, or changing the applied codes to lines or excerpts. At the end of this step, the number of labels became 29 in 5 categories.

With the new codebook, the first two authors re-annotated 10 
 of the previous 20 answers and confirmed the agreement. %They regrouped to review the annotations and identify new conflicts. At this meeting, 
 Except for one disagreement about the definition and usage of one code, no new disagreement was discovered. \new{At this point, Fleiss's Kappa \todo{cite} score is 0.79 and Krippendorff's Alpha \todo{cite} is 0.67.} %The two authors revisited the annotations and codebook and carefully re-defined those codes to resolve this conflict. 

Next, the first two authors met the co-author to review and refine the current codebook and annotations. 
%A new conflict on using a separate codebook for code answers arise in this meeting. The three authors disputed that by reviewing ChatGPT answers with code and decided to use a separate codebook for annotating the coding parts of ChatGPT answers.
At the end of this meeting, a second Codebook (Codebook \ref{tab:codebook2}) with 4 codes was created for annotating Codes embedded in ChatGPT answers. The original Codebook (we will call it Codebook \ref{tab:codebook1}) was refined to 27 labels.  

Finally, the first two authors annotated 10 new ChatGPT answers with the new cookbook and found there were very few disagreements that were more subjective in nature (e.g. usefulness).  \new{At this point, Fleiss's Kappa score is 0.83 and Krippendorff's Alpha is 0.80.}
With this codebook, the first two authors annotated \todo{XX} ChatGPT answers. The whole labeling process took about \todo{YY} man-hours. 

\begin{table}
  \caption{Codebook for annotating Text Answers generated by ChatGPT }
  \label{tab:codebook1}
  % \resizebox{0.5\textwidth}{!}{
    \begin{tabular}{cl}
        \toprule
        Category & Codes\\
        \midrule
        Correctness & Correct \\  & Incorrect (Factual) 
    \\  &Incorrect (Code) 
    \\  &Incorrect (Concept) 
    \\  &Incorrect (Terminology) 
    \\  &Incorrect (Irrelevant) \\
                      
        \midrule
         Consistency & Consistent \\  & Inconsistent (Factual) 
    \\  &Inconsistent (Code) 
    \\  &Inconsistent (Concept) 
    \\  &Inconsistent (Terminology) 
    \\  &Inconsistent (Irrelevant) 
    \\  &Inconsistent (Number of solutions) \\
        \midrule
    
         Comprehensiveness  & Comprehensive  \\ & Partially Comprehensive 
    \\ & Not Comprehensive \\
        \midrule
    
         Conciseness  & Concise  \\ & Not Concise (Redundant) 
    
        \\ &Not Concise (Unnecessary) 
        
        \\ &Not Concise (Overlapping steps) 
        
        \\ &Not Concise (Missing examples) 
        
        \\ &Not Concise (Overlapping segments)  \\
            \midrule
    
         Usefulness  & Useful (1)  \\ & Useful (2) \\ & Useful (3) \\ & Useful (4) \\ & Useful (5) \\
         
        \bottomrule
    \end{tabular}
% }
\end{table}



\begin{table}
  \caption{Codebook for annotating Code Answers generated by ChatGPT }
  \label{tab:codebook2}
  % \resizebox{0.5\textwidth}{!}{
  \begin{tabular}{cl}
    \toprule
    Category & Codes\\
    \midrule
    Correct &   \\ 
    \midrule
    Incorrect & Syntax Error \\ & Run-time Error 
    \\& Non-Functional \\& Implausible \\
                  
    \bottomrule
  \end{tabular}
% }
\end{table}




==> sections/todos.tex <==
% \section{ToDos}



% \todo{list atmost 3 contributions}

% \todo{layout the paper structure with headers and subheaders}

% \todo{Related works at the end}

% \todo{Dump all the research questions}

% \todo{add in the figures(Write one or two sentences of the key messages) and tables}

% \todo{Deprioritize writing texts}
